MopEye: Opportunistic Monitoring of Per-app Mobile Network Performance

Crowdsourcing mobile user's network performance has become an effective way of understanding and improving mobile network performance and user quality-of-experience. However, the current measurement method is still based on the landline measurement paradigm in which a measurement app measures the path to fixed (measurement or web) servers. In this work, we introduce a new paradigm of measuring per-app mobile network performance. We design and implement MopEye, an Android app to measure network round-trip delay for each app whenever there is app traffic. This opportunistic measurement can be conducted automatically without users intervention. Therefore, it can facilitate a large-scale and long-term crowdsourcing of mobile network performance. In the course of implementing MopEye, we have overcome a suite of challenges to make the continuous latency monitoring lightweight and accurate. We have deployed MopEye to Google Play for an IRB-approved crowdsourcing study in a period of ten months, which obtains over five million measurements from 6,266 Android apps on 2,351 smartphones. The analysis reveals a number of new findings on the per-app network performance and mobile DNS performance.

==> deploy.tex <==
\section{Crowdsourcing Deployment}
\label{sec:deploy}

We deployed \name to Google Play~\cite{MopEyeOnPlay} for a
crowdsourcing measurement study on 25 May 2016\footnote{IRB approval was obtained
  from Singapore Management University on 9 October 2015 under
  application IRB-15-093-A077(1015).}.  We make sure that all users
are consented before participation through an in-app consent form
dialog.  To make \name a long-term study, we have also created a
Facebook Page~\cite{MopEyeOnFB} to maintain \name's user community.
In the rest of this section, we show how we preserve user privacy in
the crowdsourcing study and how we handle various deployment issues.


\subsection{Preserving User Privacy}
\label{sec:privacy}

Protecting the privacy of \name users is our important design
consideration.  First, we do not collect person-identifiable
information, such as device IMEI, IP addresses, MAC addresses and fine-grained
locations.  Instead, we collect only a randomly generated
ANDROID\_ID~\cite{ANDROIDID} (hashed in SHA-1 with a secret salt),
non-sensitive phone model and OS version, and coarse-grained
locations.  Second, we use only encrypted HTTPS connections to
transmit the measurement data to our server.  Furthermore, \name's
measurement results do not include destination URLs, because \name is
not designed to analyze TCP contents like the works on detecting
privacy leakages
(e.g.,~\cite{PrivacyGuard15,Haystack15,AntMonitor15,ReCon16}).

%Furthermore, we do \textit{not} record mobile browsers' measurement results for better privacy. Unlike other apps, browsers' traffic will contain user-inputed domains. It is worth noting that, for all cases, \name's measurement results do \textit{not} include destination URLs, because \name is not designed (and thus has no capability) to analyze TCP contents like some other VPN-based academic works.


\subsection{Handling Deployment Issues}
\label{sec:realissue}

During the crowdsourcing deployment, we encountered and addressed many
deployment issues.

\textbf{Maintaining the liveness of VPN service} Keeping \name's VPN
service alive (until users explicitly close it) is necessary for a
robust long-term measurement.  However, it is non-trivial, because user
events (e.g., network switching or system restart) may disrupt the VPN
service.  To address this problem, we register Android broadcast
receivers~\cite{BroadcastReceiver} to seamlessly restart \name's VPN
service after detecting connection changes or system boots.  We
further set up a liveness monitor (that listens to a few non-frequent
system broadcasts, such as power connected events) to recover the VPN
service when it is exceptionally terminated.


\textbf{Containing network-unfriendly behaviors} As we will present in
\mysec\ref{sec:result}, we observe some apps sending a large number of
network requests in the background. These
measurement results, if all recorded, will deny our server's
service.  Therefore, we enforce three thresholds for each \name
network session to limit recording of the same error, similar DNS
records, and the same TCP connections.  We also plan to enforce
similar policies in packet relaying in the next version of \name to
help users control network-unfriendly behaviors.


\textbf{Minimizing battery consumption} While \name
collects location and signal strength information, we put extra effort
to minimize their overhead in battery consumption. For example, we
only collect the location information once for each \name session.
Moreover, we do not set up the common, but expensive, location
callback listeners~\cite{LocationStrategy}; instead, we invoke the
\texttt{getLastKnownLocation} API~\cite{getLastKnownLocation} to
estimate a coarse-grained location with negligible cost.  To collect
signal strength, we register a listener but activate it only when
\name is running under cellular networks.  When the device is
connected to WiFi, we retrieve the WiFi signal strength directly
through an API (without the listener).


\textbf{Limitations} Even though we are actively improving \name,
there are still several limitations.  First, device
fragmentation~\cite{Fragmentation} is a well-known issue, but it is not our goal
to make \name compatible with every Android 4.0+ device.
%DNS not captured on Samsung devices
Second, \name currently does not support ICMP packet relaying.
Although a related work~\cite{Haystack15} considers this issue
unsolvable (as Android does not allow apps to send customized ICMP
packets), we believe that we can achieve it in our future version by
invoking the system ping program (i.e., \texttt{/system/bin/ping}) to
recover the original ICMP packets and generating ICMP responses based
on the ping results to the VPN tunnel.  Additionally, supporting IPv6
is also underway.  Third, according to~\cite{Haystack15}, there is a
system issue that only 1,024 file descriptors can be allocated
simultaneously on Android.  \name currently mitigates this issue by
timely closing completed sockets and restarting the VPN service upon a
network switching event.
%Over the long run, we believe that this issue could be fixed by Google Android.


%We deployed \name to Google Play~\cite{MopEyeOnPlay} for a
%crowdsourcing measurement study\footnote{IRB approval was obtained
%  from Singapore Management University on 9 October 2015 under
%  application IRB-15-093-A077(1015).}.  We make sure that all users
%are consented before participation through an in-app consent form
%dialog.  To make \name a long-term study, we have also created a
%Facebook Page~\cite{MopEyeOnFB} to maintain \name's user community.
%In the rest of this section, we show how we preserve user privacy in
%the crowdsourcing study and how we handle the technical issues.
%
%
%\subsection{Preserving User Privacy}
%\label{sec:privacy}
%
%Protecting the privacy of \name users is our important design
%consideration.  First, we do not collect person-identifiable
%information, such as device IMEI, IP, MAC addresses or fine-grained
%locations.  Instead, we collect only a randomly generated
%ANDROID\_ID~\cite{ANDROIDID} (hashed in SHA-1 with a secret salt),
%non-sensitive phone model and OS version, and coarse-grained
%locations.  Second, we use only encrypted HTTPS connections to
%transmit the measurement data to our server.  Furthermore, \name's
%measurement results do not include destination URLs, because \name is
%not designed to analyze TCP contents like the works on detecting
%privacy leakages
%(e.g.,~\cite{PrivacyGuard15,Haystack15,AntMonitor15,ReCon16}).
%
%%Furthermore, we do \textit{not} record mobile browsers' measurement results for better privacy. Unlike other apps, browsers' traffic will contain user-inputed domains. It is worth noting that, for all cases, \name's measurement results do \textit{not} include destination URLs, because \name is not designed (and thus has no capability) to analyze TCP contents like some other VPN-based academic works.
%
%
%\subsection{Handling Technical Deployment Issues}
%\label{sec:realissue}
%
%During the crowdsourcing deployment, we encountered and addressed many
%deployment issues.
%
%\textbf{Maintaining the liveness of VPN service} Keeping \name's VPN
%service alive (until users explicitly close it) is necessary for a
%robust long-term measurement.  However, it is non-trivial because user
%events (e.g., network switching or system restart) may disrupt the VPN
%service.  To address this problem, we register Android broadcast
%receivers~\cite{BroadcastReceiver} to seamlessly restart \name's VPN
%service after detecting connection changes or system boots.  We
%further set up a liveness monitor (that listens to a few non-frequent
%system broadcasts, such as power connected events) to recover the VPN
%service when it is exceptionally terminated.
%
%
%\textbf{Limiting the records of network-unfriendly behaviors} As we will present in
%\mysec\ref{sec:result}, we observe some apps sending a large number of
%network requests in the background. These
%measurement results, if all recorded, will deny our server's
%service.  Therefore, we enforce three thresholds for each \name
%network session to limit recording of the same error, similar DNS
%records, and the same TCP connections.  We also plan to enforce
%similar policies in packet relaying in the next version of \name to
%help users control network-unfriendly behaviors.
%
%
%\textbf{Minimizing battery consumption} While \name
%collects location and signal strength information, we put extra effort
%to minimize the corresponding overhead in battery consumption.  We
%only collect the location information once for each \name session.
%Moreover, we do not set up the common, but expensive, location
%callback listeners~\cite{LocationStrategy}; instead, we invoke the
%\texttt{getLastKnownLocation} API~\cite{getLastKnownLocation} to
%estimate a coarse-grained location with negligible cost.  To collect
%signal strength, we register a listener but activate it only when
%\name is running under cellular networks.  When the device is
%connected to WiFi, we retrieve the WiFi signal strength directly
%through an API (without the listener).
%
%
%\textbf{Limitations} Even though we are actively improving \name,
%there are still several limitations.  First, device
%fragmentation~\cite{Fragmentation} is a well-known issue and we do not
%strike to make \name compatible with every Android 4.0+ device.
%%DNS not captured on Samsung devices
%Second, \name currently does not support ICMP packet relaying.
%Although a related work~\cite{Haystack15} considers this issue
%unsolvable (as Android does not allow apps to send customized ICMP
%packets), we believe that we can achieve it in our future version by
%invoking the system ping program (i.e., \texttt{/system/bin/ping}) to
%recover the original ICMP packets and generating ICMP responses based
%on the ping results to the VPN tunnel.  Additionally, supporting IPv6
%is also underway.  Third, according to~\cite{Haystack15}, there is a
%system issue that only 1,024 file descriptors can be allocated
%simultaneously on Android.  \name currently mitigates this issue by
%timely closing completed sockets and restarting the VPN service upon a
%network switching event.
%%Over the long run, we believe that this issue could be fixed by Google Android.


==> discuss.tex <==
\section{Discussion}
\label{sec:discuss}

In this section, we discuss the position of \name in light of other works that also use the \texttt{VpnService} API, as well as future analysis of our crowdsourcing dataset.


\name is the first and the only one in its kind that provides per-app measurement for end users.
By the time of our submission, there are still no any other VPN-based apps achieving the same goal.
This novelty lays the major difference between our paper and the aforementioned related works.
Additionally, we are among the first batch of several studies~\cite{AntMonitor15, PrivacyGuard15} that leverage the \texttt{VpnService} API---we started the \name project two years ago and submitted the first version of \name in May 2015, followed by a published poster~\cite{MopEyePoster15}.
%TODO Do we need the following as like SigCOMM15_Encore?
%We started the \name project two years ago and submitted the first version of \name to IMC'15.
%We then significantly optimized \name's performance and published a two-page poster~\cite{MopEyePoster15} in CoNEXT'15.


Although we have presented the first study of large-scale per-app measurements in \mysec\ref{sec:tcpresult}, there are more analysis we can do in future works.
First, our current analysis largely relies on manual efforts and are thus not scalable, we expect a technique that can generate meaningful performance reports automatically.
We are exploring this idea by proposing differential analysis algorithms.
Second, our dataset contains not only RTTs but also a large number of traffic characteristics, an analysis of which will be useful.
Third, our analysis of DNS measurements in \mysec\ref{sec:dnsresult} does not involve the impact of different DNS query payloads, and a payload-aware DNS performance analysis, like~\cite{CellDNS14}, will be interesting.


%In this section, we discuss the position of \name in light of other works that also use the \texttt{VpnService} API, as well as future analysis of our crowdsourcing dataset.
%
%
%\name is the first and the only one in its kind that provides per-app measurement for end users.
%By the time of our submission, there are still no any other VPN-based apps achieving the same goal.
%This novelty lays the major difference between our paper and the aforementioned related works.
%Additionally, we are among the first batch of several studies~\cite{AntMonitor15, PrivacyGuard15} that leverage the \texttt{VpnService} API---we started the \name project two years ago and submitted the first version of \name in May 2015, followed by a published poster~\cite{MopEyePoster15} in ACM CoNEXT'15.
%%TODO Do we need the following as like SigCOMM15_Encore?
%%We started the \name project two years ago and submitted the first version of \name to IMC'15.
%%We then significantly optimized \name's performance and published a two-page poster~\cite{MopEyePoster15} in CoNEXT'15.
%
%
%Although we have presented the first study of large-scale per-app measurements in \mysec\ref{sec:tcpresult}, there are more analysis we can do in future works.
%First, our current analysis largely relies on manual efforts and are thus not scalable, we expect a technique that can generate meaningful performance reports automatically.
%We are exploring this idea by proposing differential analysis algorithms.
%Second, our dataset contains not only RTTs but also a large number of traffic characteristics, an analysis of which will be useful.
%Third, our analysis of DNS measurements in \mysec\ref{sec:dnsresult} does not involve the impact of different DNS query payloads, and a payload-aware DNS performance analysis, like~\cite{CellDNS14}, will be interesting.






%Although the performance of the current \name is already quite good, we can further improve it, particularly for minimizing the single-round latency of SYN-ACK and data packets.
%For example, we will explore a socket pool mechanism to reduce the socket initialization time before each SYN packet.
%Similarly, we will try a thread pool mechanism to mitigate the overhead of creating each \texttt{socket-connect} thread.
%For data packets, we will explore a mechanism to reduce the read/write event notification overhead.
%In addition to the throughput enhancement, we plan to support the TCP window scale option as discussed in \mysec\ref{sec:tunetcp}.
%
%
%More functionalities can be added to the current \name prototype.
%First, we plan to allow users to filter the apps that they do not want to monitor by calling the \texttt{addDisallowedApplication()} API.
%Second, we will support the DNS payload analysis to recover the domain name of each destination IP directly on smartphones.
%Third, implementing the ICMP packet relaying is also underway.
%Although Android does not allow apps to send custom ICMP packets, we can invoke the system ping program (i.e., \texttt{/system/bin/ping}) to recover the original ICMP packets and generate ICMP responses based on the ping results to the VPN tunnel.







%Other improvements include
%(i) automatically correlating network providers and context information (e.g., locations),
%(ii) supporting ICMP and IPv6 traffic,
%and (iii) supporting the TCP/IP options and the server-initiated traffic.
%
%
%Moreover, we plan to support more measurement metrics besides the current \texttt{SYN-ACK} based RTT measurement.
%For example, we have shown in \S\ref{sec:result} that \name has the capability of detecting nonresponsive servers.
%In the next version, we will provide this feature directly to users instead of a off-line analysis.
%Furthermore, we will explore how to leverage the data traffic for more real-time RTT measurement and throughput analysis.
%Monitoring mobile DNS performance by analyzing the UDP traffic is also underway.



%Although \name currently runs on Android, it could be extended to other platforms, because its underlying packet capturing technique based on the \texttt{TUN} virtual network device has been supported on Linux/UNIX-based systems for over 15 years \cite{tuntap}.
%The popular OpenVPN~\cite{openvpnHome}, which also uses the \texttt{TUN}-based packet capturing, supports iOS without jailbreaking the device \cite{privatetunnelvpn, openvpnconnect}.
%Indeed, Apple has provided the \texttt{TUN}-based VPN API as a private API since iOS 4.2~\cite{iOSVPNAPI} and recently released it as a public API through the network extension framework on iOS 8~\cite{programIOSVPN}.
%%Hence, we envison that \name can also be implemented on iOS, thus covering the two mainstream platforms.
%%However, iOS may have some unique challenges that do not occur on Android, such as that iOS generally does not allow background server behavior \cite{MoST15}. We will try to address them when we develop the iOS version of \name in our future work.
%%Nevertheless, our current prototype on Android can already support billions of Android devices.
%
%
%
%In addition, Haystack~\cite{Haystack15} mentions a limited file descriptor issue on Android.
%But this issue is essentially an Android system bug \cite{issue39002} and seems only occurs on low versions of Android such as Android 2.3.4 and 4.1 \cite{issue39002}.


==> failedres.tex <==
\subsubsection{Measurement Failure Analysis}
\label{sec:failedresult}


Out of the 4,560 TCP connection failures, 2,695 are \texttt{SocketTimeoutException}, whereas the remaining 1,865 are \texttt{ConnectException}.
We present three case studies below to highlight \name's capability of diagnosing failures.

\begin{compactitem}
\item [\textbf{Network-unfriendly behavior:}]
We find that the LeanCloud mobile SDK~\cite{LeanCloud} used by many popular iOS and Android apps~\cite{LeanCloudUsers} will be trapped in a loop when its TCP connections to \url{router.g0.push.leancloud.cn} fail.
  That is, even if its earlier connections fail, the LeanCloud SDK will keep retrying frequently.
  As a result, lots of TCP connections and DNS queries are issued in a short period of time, leading to significant network usage and battery consumption.
  %We are on the way of contacting LeanCloud to address this serious software bug.
  Furthermore, the LeanCloud failures occur in a WiFi network of Starhub, a Singapore ISP, but not in Singtel-based WiFi and cellular networks.
  This indicates that some network paths to the LeanCloud server also have problems, which is confirmed recently by an online post~\cite{LeanCloudError} in the LeanCloud forum.


\item [\textbf{A case study of \texttt{ConnectException}:}]
To illustrate the \texttt{ConnectException}, we use Sina Weibo's \url{gw5.push.mcp.weibo.cn:4828}, which has a total of 238 refused connections in SMU WiFi.
Interestingly, there are also 341 successful connections under the same network.
By analyzing the destination IP addresses, we find that the successful connections are all connected to \texttt{180.149.153.100}, a Weibo server in Beijing, whereas the failed connections are mapped to six IP addresses in Hong Kong (\texttt{183.91.33.41/42/43/44} and \texttt{183.91.33.74/75}), which most likely are not Weibo servers.
Moreover, we find that the mis-mapped IP addresses occur only in SMU WiFi, but not other Singapore-based WiFi or cellular networks.
These findings make us believe that Weibo's failures are due to errors in SMU WiFi's DNS service.


\item [\textbf{A case study of \texttt{SocketTimeoutException}:}]
  %--Written by Weichao--(need to be in one paragraph)
  The second example is Netease News app, the most popular news app in China, which encounters extremely large network delay, especially to the server \url{news.push.126.net}. The mean RTT to this news server is more than 440ms, whereas that for other servers is only $\sim$275ms. The measurement logs show that the app generates 140 error records, half of which are triggered by the news server. Our further analysis shows that more than 97\% of the errors are due to TCP connection timeout. As the remaining errors come from 68 different servers ($\sim$1 event for each), we can conclude that the news server accounts for the majority of the errors.
  %We further perform measurement in desktop environment to validate this observation. We resolve the domain name of the news server and get the same IP address to the mobile environment. Our ping measurement results to this IP show that the packet loss rate can be as high as 16\%, which confirms that the performance bottleneck could be the news server or the network links close to the server.
  Our ping measurement results to the IP address of this news server show that the packet loss rate can be as high as 16\%, thus confirming that the performance bottleneck could be the news server or the network links close to the server.
\end{compactitem}



%\noindent
%\red{
%- Network-unfriendly (That mobile SDK)\\
%- Only ConnectionException: pingable or unpingable\\
%- Larger RTT: mostly TimeoutException\\
%- DNS configuration errors (The poster version)\\
%}
%
%
%\noindent
%\red{
%- Then case study representative failure cases:\\
%++ (The example for ConnectionException) WeChat's dispatcher.3g.qq.com, no successful RTT log. Are were rejected, but its IP (103.7.31.184) is pingable\\
%++ Facebook's edge-mqtt.facebook.com, mqtt-mini.facebook.com\\
%++ Google's mtalk.google.com for Google Play services (com.google.android.gms) and google services framework (com.google.android.gsf). But maybe this is XiaoMi's problem\\
%++ Sina Weibo's gw5.push.mcp.weibo.cn\\
%++ Alipay (com.eg.android.AlipayGphone)'s 326 error logs. In particular, 198.11.148.99 (port 443)\\
%++ (Example for larger RTT, especially for dlink-541C starhub network) Netease News's news.push.126.net\\
%++ XiaoMi phone\\
%}

